Grounded Copilot: How Programmers Interact with Code-Generating Models

Powered by recent advances in code-generating models, AI assistants like Github Copilot promise to change the face of programming forever. But what is this new face of programming? We present the first grounded theory analysis of how programmers interact with Copilot, based on observing 20 participants--with a range of prior experience using the assistant--as they solve diverse programming tasks across four languages. Our main finding is that interactions with programming assistants are bimodal: in acceleration mode, the programmer knows what to do next and uses Copilot to get there faster; in exploration mode, the programmer is unsure how to proceed and uses Copilot to explore their options. Based on our theory, we provide recommendations for improving the usability of future AI programming assistants.

==> conclusion.tex <==
\section{Conclusion}

\subsection{Underexplored Phenomena}
\mjsays{Maybe we should have a subsection like this?}
\subsubsection{}


\subsection{Future Work}
The majority of research in machine learning, programming languages, and
human-computer interactions happen in English.
%
While we do not know if Github and Microsoft did anything extra to aid English as
a second language (ESL) programmers, we do know that the majority of the code
their model is trained on, is in English \mjsays{Citation needed}.
%
Some participants seem keenly aware that the language they think in differs from
what Copilot was largely trained on, with P14 noting, ``it doesn't feel
as natural to me''\mjsays{P14@1:13:00}.
%
P14 was hesitant to write comments, citing a language barrier as an added hurdle
(in addition to just typing out a comment) to being able to save time by using
Copilot.
%
For research in neurally-guided program synthesis to be equitable, tools should
be better trained on non-English language.
%
A future study might directly look at the impact of different English-language
abilities or non-English languages on the types of input provided to tools like
Copilot \mjsays{that was garbage, and I'm sorry you had to read that.}.

A few participants mentioned that the natural language interaction mode of Copilot felt natural to them because it helped them think out loud, lay down the architecture TODOs in natural language to get a high-level picture before starting to code. However P14 pointed out that they are a visual learner so they prefer to draw design diagrams/flowcharts as opposed to writing text. It would be interesting to conduct a more directed study on how and when people find it natural to write comments. Also, if there was a more visual mode of interaction with Copilot in addition to natural language, that would be inclusive of visual learners workflow as well.



